The SKIM-FA Kernel: High-Dimensional Variable Selection and Nonlinear Interaction Discovery in Linear Time

Many scientific problems require identifying a small set of covariates that are associated with a target response and estimating their effects. Often, these effects are nonlinear and include interactions, so linear and additive methods can lead to poor estimation and variable selection. Unfortunately, methods that simultaneously express sparsity, nonlinearity, and interactions are computationally intractable -- with runtime at least quadratic in the number of covariates, and often worse. In the present work, we solve this computational bottleneck. We show that suitable interaction models have a kernel representation, namely there exists a "kernel trick" to perform variable selection and estimation in $O$(# covariates) time. Our resulting fit corresponds to a sparse orthogonal decomposition of the regression function in a Hilbert space (i.e., a functional ANOVA decomposition), where interaction effects represent all variation that cannot be explained by lower-order effects. On a variety of synthetic and real data sets, our approach outperforms existing methods used for large, high-dimensional data sets while remaining competitive (or being orders of magnitude faster) in runtime.

==> algos_moved.tex <==
 \begin{algorithm}[H]
    \caption{Learn SKIM-FA Kernel Hyperparameters and Kernel Ridge Weights}
    \label{algo:learn_skim_hyp}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        %\Procedure{LearnHyp}{$D$, $Q$, $c$, $\{k_i\}_{i=1}^p$, $M$, $\gamma$, $T$} where $D$ equals the observed data, $Q$ the highest order effect,  $c$ cutoff in ADD REF, $\{k_i\}_{i=1}^p$ univariate mean-zero kernels, $M$ the cross-validation fold size, $\gamma$ the learning rate, $T$ the number of gradient descent steps 
         \Procedure{LearnHyperParams}{$M$, $\gamma$, $T$} %$M$ the cross-validation fold size, $\gamma$ the learning rate, $T$ the number of gradient descent steps 

		\State For all $i  \in [p]$, set $\tilde{U}_i^{(0)} = 1$, $\eta^{(0)} = [1, \cdots, 1]^T \in \R^{Q+1}$
		
		%\State $\eta^{(0)} = [1, \cdots, 1]^T \in \R^Q$
		
		\State $\sigma^{(0)}_{\text{noise}} = \sqrt{0.5\var(Y)}$ \Comment{Initialize noise variance as half of the response variance}
		
		\State $\tau^{(0)} = (\tilde{U}^{(0)}, \eta^{(0)},\sigma^{(0)}_{\text{noise}})$

            \For{$t \in 1:T$} \Comment{Update parameters via gradient descent}
            		\State{Randomly select $N-M$ datapoints and collect  covariates and responses in $X_A$, $Y_A$}
				
				\For{$i \in 1:p$}            		
            		
            		%\State $U_i^{(t)} = \frac{[\tilde{U}_i^{(t)}]^2}{[\tilde{U}_i^{(t)}]^2 + 1}$
            		
            		\State $\kappa_i^{(t)} = \max\left( \frac{[\tilde{U}_i^{(t)}]^2}{[\tilde{U}_i^{(t)}]^2 + 1} - c, 0\right)$
				            		
            		
            		 \EndFor
            		
            		\State Compute kernel matrix $K_{\tau}^A$, where $[K_{\tau}^A]_{ij} = k_{\text{SKIM-FA}}(X^A_i, X^A_j)$ via \cref{eq:skim_fast_form}
            		
            		\State Let $f_A$ equal the solution of \cref{eq:kern_ridge} with $\lambda = [\sigma^{(t)}_{\text{noise}}]^2$, $K = K_{\tau}^A$, $Y = Y_A$
            		
            		\State $L = \frac{1}{M} \sum_{n \in [N] \setminus A} (y^{(n)} - f_A(x^{(n)}))^2$
            		
            		\State $\tau^{(t)} = \tau^{(t-1)}  - \gamma \nabla_{\tau^{(t-1)}} L$ \Comment{Compute
gradients with automatic differentiation}
            		            		               
            \EndFor 
            
            \State Compute $\alpha^{(T)}$, the kernel ridge regression weights found by solving \cref{eq:kern_ridge} using all $N$ datapoints with SKIM-FA hyperparameters equal to $\kappa^{(T)}, \eta^{(T)}, \sigma^{(T)}_{\text{noise}}$
                                 
            \State \textbf{return} $\kappa^{(T)}, \eta^{(T)}, \sigma^{(T)}_{\text{noise}}, \alpha^{(T)}$
            
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

 \begin{algorithm}[H]
    \caption{SKIM-FA Variable Selection}
    \label{algo:var_select}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        %\Procedure{LearnHyp}{$D$, $Q$, $c$, $\{k_i\}_{i=1}^p$, $M$, $\gamma$, $T$} where $D$ equals the observed data, $Q$ the highest order effect,  $c$ cutoff in ADD REF, $\{k_i\}_{i=1}^p$ univariate mean-zero kernels, $M$ the cross-validation fold size, $\gamma$ the learning rate, $T$ the number of gradient descent steps 
         \Procedure{VarSelect}{$\kappa$}
            \State \textbf{return} $ \{i: \kappa_i \neq 0 \} $
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

 \begin{algorithm}[H]
    \caption{Estimated functional ANOVA effect $\bar{f}_V$ of $\bar{f}_{\theta}$ with respect to $\mu_{\tens}$}
    \label{algo:orth_effects}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        %\Procedure{LearnHyp}{$D$, $Q$, $c$, $\{k_i\}_{i=1}^p$, $M$, $\gamma$, $T$} where $D$ equals the observed data, $Q$ the highest order effect,  $c$ cutoff in ADD REF, $\{k_i\}_{i=1}^p$ univariate mean-zero kernels, $M$ the cross-validation fold size, $\gamma$ the learning rate, $T$ the number of gradient descent steps 
         \Procedure{OrthEffects}{$V$, $\alpha$, $\kappa$, $\eta$, $\alpha$} %where $\alpha$ equals the fitted kernel ridge regression weights

		\State $\theta_V = \eta_{|V|}^2 \prod_{i \in V} \kappa_i^2$
                      
            \State \textbf{return} $\bar{f}_V(\cdot) = \theta_V \sum_{n=1}^N \alpha_n k_V(x^{(n)}, \cdot)$ 
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
    \caption{Change of Basis Formula for Finite Dimensional Model Selection Kernels}
    \label{algo:change_basis}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
         \Procedure{ReExpressEffect}{$\alpha$, $k_{\theta}$, $W$, $\mu$}  
         	\State Compute $ f_{\{ i, j \}}^{\mu_{\tens}} , f_{\{ i \}}^{\mu_{\tens}}, f_{\emptyset}^{\mu_{\tens}}$ using \cref{algo:orth_effects}
			\State For $1 \leq w \leq W$ randomly sample $x^{(w)} \iid \mu$     
			\State Compute $X_{ij} = [\Phi_i(x^{(1)}_i) \cdots \Phi_i(x^{(W)}_i) \ \Phi_j(x^{(1)}_j) \cdots \Phi_j(x^{(W)}_j)]^T$
			\State Compute  $f_{ij, W}^{\mu_{\tens}} = [f_{\{ i, j \}}^{\mu_{\tens}}(x^{(1)}_i,  x^{(1)}_j) \cdots f_{\{ i, j \}}^{\mu_{\tens}}(x^{(W)}_i,  x^{(W)}_j)]^T$
			\State Compute $[\hat{\Psi}_{ij}^i \ \hat{\Psi}_{ij}^j]^T = (X_{ij}^T X_{ij})^{-1} X_{ij}^T f_{ij, W}^{\mu_{\tens}}$ \Comment{Least-squares projection}
			\State Compute $\hat{f}_{\{ i, j \}}^{\mu} =  f_{\{ i, j \}}^{\mu_{\tens}} - [\hat{\Psi}_{ij}^i \Phi_i^T(\cdot) +  \hat{\Psi}_{ij}^j \Phi_j^T(\cdot) + \Psi_{ij}^{0}]$
			\State Compute $\hat{f}_{\{ i \}}^{\mu} =f_{\{ i \}}^{\mu_{\tens}} + \sum_{j > i} \hat{\Psi}_{ij}^i \Phi_i(\cdot) + \sum_{j < i} \hat{\Psi}_{ji}^{i} \Phi_i(\cdot)$ 
			\State Compute $\hat{f}_{\emptyset}^{\mu} = f_{\emptyset}^{\mu_{\tens}} + \sum_{i < j} \hat{\Psi}_{ij}^{0}$
            \State \textbf{return} $\hat{f}_{\{ i, j \}}^{\mu}, \hat{f}_{\{ i \}}^{\mu}, \hat{f}_{\emptyset}^{\mu} $
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> fanova_problem_setup.tex <==
 % !TEX root =  main.tex
\noindent \textbf{Non-Linear Estimation via the Functional ANOVA.}
The functional ANOVA extends this intuitive idea of breaking a function into simpler parts by incorporating higher-order interactions. This enables the functional ANOVA to model arbitrary smooth functions. It handles the issue of the identifiability by assuming that higher order effects represent all variation that cannot be explained by lower-order effects. %more "complicated" functions (i.e., those that depend on more variables) only model variation that cannot be explained by simpler functions. In other words, complicated functions are, in some mathematical sense, "orthogonal" to simpler functions. This property turns out to make simpler functions favored (a priori) over more complicated functions in the decomposition of $f^*$ and results in a well-defined inference task.
Since the decomposition depends on a notion of variance and orthogonality, the functional ANOVA begins by assuming $f^*$ belongs to the space all square-integrable measurable functions $L^2(\mu)$ with inner product
%
\begin{equation*}
	\inner{f}{g}_{\mu} \coloneqq \int_{x \in \R^p} f(x)g(x)d\mu(x), \qquad 	\| f \|^2_{\mu} \coloneqq  \inner{f}{f}_{\mu},
\end{equation*}
%
where $\mu$ is some arbitrary probability measure.
%The induced norm from this choice of inner product is
%\begin{equation*}
%	\| f \|^2_{\mu} =  \inner{f}{f}_{\mu}.
%\end{equation*}
%
Two functions $f$ and $g$ are "orthogonal" when their inner product is zero, which we denote by $\indep_{\mu}$ to emphasize that this notion of orthogonality depends intimately on the chosen measure:
%
\begin{equation}
	f \indep_{\mu} g \iff \inner{f}{g}_{\mu} = 0.
\end{equation}
%
Since $\inner{f}{g}_{\mu}$ can be written as $\E_{x \sim \mu}[ f(x) g(x)]$, $\inner{f}{g}_{\mu}$ measures the dependence between functions through their covariance. Therefore, we use the notation $\cov(f, g)$ and $\inner{f}{g}_{\mu}$ interchangeably. Similarly, we use $\var(f) = \cov(f, f)$ and $	\| f \|^2_{\mu}$ interchangeably.

Given some additional mild technical conditions about $\mu$ and $\hilb$ (see Section 3 of \cite{projection_anova}), the \emph{hierarchical functional ANOVA} \citep{stone1994} uniquely decomposes any $f \in L^2(\mu)$ as 

%
\begin{equation}
	f(x) = \sum_{V \in 2^{[p]}} f_V(x), \ f_V \in L^2(\mu) \quad \text{s.t.} \quad \frac{\partial f_V(x)}{\partial x_{V^c}} = 0   \\
\end{equation}
%
under the \emph{hierarchical orthogonality constraints}
\begin{equation} \label{eq:hier_orth_constraints}
	f_A \indep_{\mu} f_{B} \ \ \forall A \subset B \in 2^{[p]}, \ A \neq B,
\end{equation}

where $[p] \coloneqq \{1, \cdots, p\}$. Since $f_V$ does not functionally depend on variables outside of $V$ by the derivative constraint, we may re-write each $f_V$ as a function of just the variables $\{x_v\}_{v \in V}$. After re-arranging terms in \cref{eq:hier_orth_constraints}, $f$ reduces to a sum of functions that depend on more and more variables (i.e., growing complexity):

\begin{equation} \label{eq:fanova_expansion}
	f(x) = \underbrace{f_{\{\emptyset\}}}_{\text{"Intercept"}} + \underbrace{\sum_{i} f_{\{i\}}(x_i)}_{\text{"One-Way Effects"}} + \underbrace{\sum_{i, j} f_{\{i,j\}}(x_i, x_j)}_{\text{"Two-Way Effects"}} + \cdots +  \underbrace{f_{\{1,2, \cdots, p\}}(x_1, \cdots, x_p)}_{\text{"$p$-Way Effects"}}, \\
\end{equation}

where $f_V \in L^2(\mu_V)$ and $\mu_V$ equals the marginal distribution of $x_V$ with respect to $\mu$; see also, \citet{projection_anova, stone1994}.
%Denoting $\hilb_i$ as the Hilbert space of 1D functions of $x_i$, there always exists $\hilb_i$ such that each term $f_{V}$ in \cref{eq:fanova_expansion} belongs to $\bigotimes_{i \in V} \hilb_i $; see \TODO{add ref}. Hence, 
%%
%\begin{equation}
%	\hilb = \bigoplus_{V \in 2^{[p]}} \left[ \bigotimes_{i \in V} \hilb_i \right]
%\end{equation}
%%
By the orthogonality constraints, $f_{\{i,j\}}(x_i, x_j)$ represents, for example, the variation that cannot be explained by 1D functions of $x_i$ and $x_j$ and an intercept. When $\mu$ is product measure, then the signal variance further decomposes as 
%
\begin{equation} \label{eq:sig_var_decomp}
	\begin{split}
		\var(f) = \var(f_{\{\emptyset\}}) + \sum_{i} \var( f_{\{i\}}) + \sum_{i, j} \var( f_{\{i, j\}}) + \cdots \var(f_{\{1,2, \cdots, p\}}(x_1, \cdots, x_p)),
	\end{split}
\end{equation}
%
which allows us to \emph{analyze} how the \emph{variance} of the \emph{function} is distributed across the interactions of different orders. Hence, the name functional analysis of variance or ANOVA. 

This decomposition also highlights how the functional ANOVA naturally handles model mispecification. If we only model interactions up to order $q$, then the effective noise variance $\sigma^2_{eff} = \sigma^2_{noise} + \sum_{|V| > q} \var(f_{V})$, where the first term $\sigma^2_{noise} = \var(\epsilon)$ represents unavoidable  measurement error while the second term results from mispecification. Hence, $ \sum_{|V| > q} \var(f_{V})$ quantifies the price paid for using a misspecified model in a mean-squared prediction error sense. \\

%This is the common case in traditional instantiation of fanova until generalized in \TODO{add ref} for general measuers. Below, we first show other choices of measure and discuss some issues with assuming product measure. \TODO{add Hooker ref} already showed for other data distribution.

\noindent \textbf{Resulting inference task.} Since each function admits a unique expansion under the constraints in \cref{eq:hier_orth_constraints}, we have a well-defined estimation task. One prominent method for learning the components of $f^*$ of order at most $q$ is by minimizing the penalized log-likelihood:
%
\begin{equation} \label{eq:penalized_log_like}
\begin{split}
& \min_{f \in \hilb} \frac{1}{N} \sum_{n=1}^{N} \loglike(y^{(n)}, f(x^{(n)}) + J(f) \\
										& \quad \text{s.t.} \quad f = \sum_{V \in 2^{[p]}} f_V, \quad |V| \leq q \\
										& \qquad \quad f_A \indep_{\mu} f_{B} \ \ \forall A \subset B,  \ A \neq B \\
										& \qquad \quad f_V \in L^2(\mu_V),
\end{split} 
\end{equation}
%
where $J(f)$ is some penalizer (or prior) and $\loglike$ is the log-likelihood. In this paper, our focus is on the Gaussian case, i.e., when $\loglike(y, f(x)) =(y - f(x))^2$. %We discuss extensions of our method to general exponential family likelihoods in \cref{A:model_extensions}.  %Bayesian inference can be used in a similar fashion to put a distribution over each $f_V$, where the hierarchical orthogonality constraints turn into constraints on the prior instead. 
In the next section, we discuss the statistical and computational challenges for learning such a decomposition in practice.

%existing frequentist and Bayesian methods for learning  functional ANOVA decompositions. We put an emphasis on the limitations of current methods to better contextualize our key contributions within the large body of existing work (which dates all the way back to the mid 1980s).

%ISSUE HERE IS $f_V$ SHOULDNT have independent prior. Intertwined in high-dim case.
%
%STATE HERE RELATED WORK
%
%effectively nuisance parameter that might not be expanded. In orthogonal measure case, can throw away this param and still learn components
%
%These constraints are crucial for identifiability or uniqueness of the expansion and interpretability. \TODO{explain why}
%
%As a preview, we can already see why functional ANOVA decomposition is computationally challenging on face of it; there are $2^p$ terms to fully expand! Before we outline how we deal with this computational issue with the help of a kernel trick, we keep discussing stuff.
%
%
%
%
%\textbf{Fitting the Fit.} Write the measure here. Typically, can actually do this exactly because of recursive high-dim integrals. So use some lower order 
%
%\textbf{Selecting the "Interpretable" Space for Inference.}
%
%Say either case, it's really the same question of how to actually find the decomposition. In first scenario, have $f$ and need to decompose somehow into interpretable parts. Second you have noisy evals of $f$ and want to both est. $f$ and decompose it so effectively special noise-free case (i.e., when $y = f(x)$.) Hence, it suffices to handle this second problem and what we do.  
%
%\TODO{MOVE THIS IN NEXT SECTION FOR HIGHLIGHTING ISSUE OF PRODUCT MEASURE}
%
%\textbf{Choice of Measure.} Since each choice of $\mu$ leads to a different expansion of a partiular $f$ in \TODO{add ref}, an immediate question is what $\mu$ to select? 
%
%
%We provide three examples below.
%
%\begin{itemize}
%	\item $\mu_{obs}(x) \coloneqq P(x_1, \cdots, x_p)$
%	\item $\mu_{prod}(x) \coloneqq \mu_1(x_1) \tens \mu_2(x_2) \tens \cdots \tens \mu_p(x_p)$
%	%\item $\mu_{local}(x) \coloneqq \mu(\|x^* - x\|)$
%	\item $\mu_{N}(x) := \frac{1}{N} \sum_{n=1}^N \delta_{x^{(n)}}(x)$
%\end{itemize}
%
%\TODO{PUT PIC SHOWING DIFFERENCE}
%
%\begin{nlem} \label{lem:arb_far_intercept}
%For any $\Delta \in \R^+$, there exists a probability measure $\mu_{obs}$ and $f \in L^2(\mu_{obs})$ such that the relative difference
%%
%\begin{equation}
%	\frac{| f_{\{\emptyset\}}^{\mu_{obs}} - f_{\{\emptyset\}}^{\mu_{prod}} |}{ |f_{\{\emptyset\}}^{\mu_{obs}}|} > \Delta, \qquad f_{\{\emptyset\}}^{\mu_{obs}} =  \E_{\mu_{obs}} f(X) \qquad f_{\{\emptyset\}}^{\mu_{prod}} =  \E_{\mu_{prod}} f(X)
%\end{equation}
%%
%where 
%\begin{equation*}
%	\int_{x_{-i}} d\mu_{obs}(x) = \int_{x_{-i}} d\mu_{prod}(x). 
%\end{equation*}
%\end{nlem}
%
%\cref{lem:arb_far_intercept} shows that the intercepts between two different functional ANOVA decompositions can be arbitrarily far away if we approximate the joint distribution with product measure, even when we constrain the marginals to match. While we \cref{lem:arb_far_intercept} holds for intercepts, a similar result naturally extends to differences between (e.g., main effect / high-order interaction terms). However, this difference would need to be measured in terms of the Hilbert norm instead of absolute values.
%
%Given that the intercepts can be arbitrarily far away between $\mu_{obs}$ and $\mu_{prod}$, which decomposition should the analyst use? We argue that $\mu_{obs}$ should be used in many cases due to the resulting interpretability of the intercept. If $x \sim \mu_{obs}$, then the functional ANOVA decomposition using $\mu_{obs}$ says that the best prediction (in a mean-squared sense) without knowing $x$ in advance, is  $\E_{\mu_{obs}} f(X)$. If we instead use $\E_{\mu_{prod}} f(X)$, this interpretation no longer holds since the measure is misspecified. The same analogy holds for the higher-order terms.
%
%As we explain more later, most methods, such as those that are similar in spirit to SS-ANOVA  \TODO{Add refs} use $\mu_{prod}$ due to computational convenience. We show in \TODO{add ref} how to do the decomposition with $\mu_{obs}$. An immediate challenge, of course, is we rarely know the join distribution of the covariates, and estimating $\mu_{obs}$ is statistically very challenging for even moderate $p$. 
%
%As shown in \TODO{add ref}, however, $\mu_{obs}$ only enters in the inner product. By uniform law of large numbers results, one can make a uniform law for ; see, ADD REFS.
%%
%\begin{equation}
%	\sup_{f, g} |  \inner{f}{g}_{\mu_{N}} - \inner{f}{g}_{\mu_{obs}} |
%\end{equation}
%%
%Hence, we can avoid the need to explicitly estimate $\mu_{obs}$ by computing the inner products with respect to empirical measure and by \TODO{add ref}. For each specific $f, g$, this convergence will be the standard $N^{-\frac{1}{2}}$ decay by the Law of Large Numbers. To handle the supremum over $f$ and $g$ this rate will be reduced depending on the richness of $\hilb$; see ADD REFS. While we use $\mu_{N}$ in the experiments for such reasons, our method works for arbitrary $\mu$ which we  detail in \TODO{add ref}. 
%
%%Expressing a function in terms of Hermite polynomials, wavelets, etc. are just orthogonal decompositions with different choices of measure to measure orthoginality. 
%
%%\subsection{How to Selecting Order and Non-Linearity Depends on Goals   }
%
%
%\TODO{MAKE NEW SECTIOn}
%Traditional approaches put constraints when fitting and do MLE. Show some Bayes methods anx what tthey do




==> higher_order.tex <==

%
\begin{equation} \label{eq:higher_order_skim}
	\begin{split}
	y \mid x, \Theta, \noisevar &\sim \normal(f_{\Theta}(x), \noisevar) \\
			\Theta_{V} \mid \kappa, \eta_{|V|}^2 &\sim \normal(0,  \eta_{|V|}^2 \prod_{i \in V} \kappa_i^2 \cdot I_{B^{|V|} \times B^{|V|}}) \quad |V| \leq Q \\
			\Theta_0 &\sim \normal(0, \eta_{0}^2) \\
			(\kappa, \eta^2, \noisevar) &\sim \pi_0(\kappa, \eta^2, \noisevar)
	\end{split}
\end{equation}
%

\begin{nthm} \label{thm:higher_order_skim}
The model in \cref{eq:higher_order_skim} admits an equivalent Gaussian process reparameterization:
\begin{equation}
	\begin{split}
	y \mid x, f, \noisevar &\sim \normal(f(x), \noisevar) \\
			f \mid \kappa, \eta_1^2, \eta_2^2 &\sim GP(0, k^Q_{\text{SKIM-FA}}(\cdot, \cdot)) \\
			(\kappa, \eta^2, \noisevar) &\sim \pi_0(\kappa, \eta^2, \noisevar)
	\end{split}
\end{equation}
where 
%
\begin{equation}
	\begin{split}
	& k^Q_{\text{SKIM-FA}}(x, \tilde{x}) = \sum_{q=1}^Q \eta_q^2 k_q(x, \tilde{x}) \\
	& k_q(x, \tilde{x}) = \frac{1}{q} \sum_{s=1}^q (-1)^{s+1} k_{q-s}(x, \tilde{x}) k^s(x, \tilde{x}) \\
	& k^s(x, \tilde{x}) = \sum_{i=1}^p \kappa_i^{2s} [\Phi_i(x_i)^T  \Phi_i(\tilde{x}_i)]^s
	\end{split}
\end{equation}
%
\end{nthm}

\begin{ncor}
$k^Q_{\text{SKIM-FA}}(x, \tilde{x})$ takes $O(pBQ)$ time to evaluate on a pair of points.
\end{ncor}

==> method.tex <==
 % !TEX root =  main.tex
We start by motivating a general class of hierarchical Bayesian models  that have the flexibility to encode sparsity and model non-linear effects in \cref{sec:hierch_bayes_model}. Since performing MAP inference for this class of models results in a potentially infinite-dimensional optimization problem, we convert MAP inference into a finite-dimensional one through a kernel trick in \cref{sec:model_select_kerns}.  Although a kernel trick exists, we show in \cref{sec:model_select_kerns} that the kernel is expensive to compute in general: the kernel takes $O(p^Q)$ time to evaluate on a pair of points. To remedy this computational intractability, we introduce the \emph{Sparse Kernel Interaction Model for Functional ANOVA} or \emph{SKIM-FA},  which falls within the general class of models  proposed in \cref{sec:hierch_bayes_model}. By exploiting  additional model structure in SKIM-FA, we reduce kernel evaluation time to $O(pQ)$. As a result, we show that we can estimate the functional ANOVA decomposition of $f^*$ in $O(pQN^2 + N^3)$ time by running kernel ridge regression in \cref{sec:skim_fast}. 

\subsection{Hierarchical Bayesian Model Characterization} \label{sec:hierch_bayes_model}
\noindent \textbf{Motivation.}  Suppose $f^*$ does not depend on a particular covariate $x_j$. Then, for all sets $V$ that contain covariate $x_i$, $f_V = 0$. Since we do not know a priori what covariates $f^*$ depends on, we  expect dependence between components (e.g., such as those involving covariate $x_i$). For example, if we know that $f_{1} \approx 0$ and $f_{1, 2} \approx 0$, then we might expect that $f_{1, 2, 3} \approx 0$. Unfortunately, constructing a prior (i.e., stochastic process) directly on $f_V$ that introduces dependence between the components can be difficult.  We consider a basis expansion of $f_V$ and put a prior on the basis coefficients instead. We share statistical power across different $f_V$ by placing a hierarchical Bayesian prior on the basis expansion coefficients as follows: \\

\noindent \textbf{Prior.} Assume for every $V \subset [p]$ and $1 \leq |V| \leq Q$, there exists a feature map $\Phi_V: \R^{|V|} \mapsto \R^{B_V}$ such that the components of $ \Phi_V$ form a basis of $\hilb_V^o$ in \cref{eq:orth_hilb}\footnote{In \cref{sec:model_select_kerns}, we prove that this assumption is satisfied when the base component space $\hilb_V$ is an RKHS.}. Then, for any $f_V \in \hilb_V^o$, there exists $\Theta_{V} \in \R^{B_V}$ such that $f_V(x_V) = \Theta_{V}^T \Phi_V(x_V)$. We consider the following class of models, which includes many existing sparse Bayesian regression methods as special cases (see, for example, \citet{sparse_bayes_pairwise,Curtis13fastbayesian, heirc_sparisty, kit, chipman_bayes_glm, george1993variable}):
  %
\begin{equation} \label{eq:gen_bayes_model}
	\begin{split}
			\Theta_{V} \mid \theta_{V} &\sim \normal(0,  \theta_{V} \cdot I_{B_V} \times I_{B_V}), \ V \subset [p], \ |V| \leq Q, \theta_V > 0 \\
			f_{\Theta}(x) &= \sum_{V: |V| \leq Q} \Theta_V^T \Phi_V(x) \\
				y^{(n)} \mid x^{(n)}, \Theta, \noisevar &\sim \normal(f_{\Theta}(x^{(n)}), \noisevar), \ n \in [N],
	\end{split}
\end{equation}
%
where the $\{ \theta_V \}$ can be fixed hyperparameters, or latent parameters also drawn from some prior. When $\theta \coloneqq \{\theta_V\}_{V: V \leq Q}$ is random, then \cref{eq:gen_bayes_model} enables us to encode sparsity and dependence between the $\Theta_{V}$ (and consequently the $f_V$) by encoding dependence in the components of $\theta$; see, for example, \citet{heirc_sparisty}. \\

\noindent \textbf{Computational Challenges.} Suppose, for simplicity, that there exists some $B$ such that for all $V$, $B_V = B$. Then, conditional on $\theta$, \cref{eq:gen_bayes_model} reduces to conjugate Bayesian regression. Unfortunately, computing the posterior distribution or MAP estimate of $\Theta_V$ takes $O((p^QB^Q)^{3} + (p^QB^Q)^{2} N)$ time, which is intractable for even small $p$ when $Q > 1$. Moreover, in the infinite dimensional case when $B = \infty$, the posterior is not even computatable. Fortunately, by \citet[Chapter 2]{gp_book}, there exists a Gaussian process parameterization of \cref{eq:gen_bayes_model} (and hence a potentially efficient kernel trick for inference). In the next section, we show that we can instead perform inference using \emph{model selection kernels}, which were first used in \citet{ss_anova} for the special case of independent covariates.
 
\subsection{Duality with "Model Selection Kernels"} \label{sec:model_select_kerns}

If each $\hilb_V^o$ is a reproducing kernel Hilbert space (RKHS), then there exists a positive definite kernel function such that we can instead draw $f$ from a Gaussian process prior \citep{gp_book}.  The proposition below establishes the existence of such a kernel. 
%
\begin{nprop} \label{prop:kern_exist}
(existence) Suppose $\hilb_V$ is an RKHS. Then, $\hilb_V^o$ is an RKHS. 
\end{nprop}
% 
Below, we show that \emph{model selection kernels} yield the equivalence between \cref{eq:gen_bayes_model} and the Gaussian process formulation. Then, we show how to perform variable selection and estimation after computing the posterior predictive mean of the GP.
%
\begin{ndefn} \label{def:model_select_kernel}
A kernel $k_{\theta}$ is a \emph{model selection kernel} on $\hilb$ if $k_{\theta} = \sum_{V: |V| \leq Q} \theta_V k_V$ is a reproducing kernel, where $k_V(x, \tilde{x}) = \Phi_V(x_V)^T  \Phi_V(\tilde{x}_V)$,  $\theta_V\geq 0$, and $\theta = \{ \theta_V \}_{V: |V| \leq Q}$. Furthermore, $k_{\emptyset}(x, \tilde{x}) = 1$ (i.e., the kernel that induces the space of constant functions $\hilb_{\emptyset})$.
\end{ndefn}
%
\begin{nlem} \label{prop:model_select_bayes} Suppose $k_{\theta}$ is a model selection kernel. Then, the distribution of $Y \mid x$ under \cref{eq:gen_bayes_model} equals the distribution under the following model:
%
\begin{equation*}
	\begin{split}
		f &\sim GP(0, k_{\theta}) \\
		y \mid f, x &\sim \normal(f(x), \noisevar),
	\end{split}
\end{equation*}
%
where $GP(0, k_{\theta})$ denotes a zero-mean Gaussian process with kernel function $k_{\theta}$.
\end{nlem}
%
Through the GP formulation in \cref{prop:model_select_bayes}, the posterior predictive mean $\bar{f}_{\theta}(x) \coloneqq \pr(f(x) \mid D, \theta)$ under \cref{eq:gen_bayes_model}  equals
%
\begin{equation} \label{eq:kern_ridge}
	\bar{f}_{\theta}(x) = \sum_{n=1}^N \hat{\alpha}_n k_{\theta}(x_n, x), \quad \hat{\alpha} =  (K_{\theta} + \lambda I_{N \times N})^{-1} Y,
\end{equation}
%
where $Y_n = y^{(n)}$ and $[K_{\theta}]_{nm} = k_{\theta}(x^{(n)}, x^{(m)})$. In general, it is unclear how to analytically compute the functional ANOVA decomposition of $\bar{f}_{\theta}(x)$ for arbitrary kernels. Fortunately, model selection kernels allow us to immediately recover the functional ANOVA decomposition of $\bar{f}_{\theta}(x)$ as follows: 
%
\begin{nlem}  \label{lem:kern_select}
Suppose $k_{\theta}$ is a model selection kernel and $f^{(M)}(x) = \sum_{m=1}^M \alpha_m k_{\theta}(x_m, x)$ for $\alpha_m \in \R$ and $x_m \in \R^p$. Then,  $f^{(M)}(x)  = \sum_{V: |V| \leq Q} f_V$, where $f_V =  \theta_V \sum_{m=1}^M \alpha_m k_{V}(x_m, x) \in \hilb_V^o$.
\end{nlem}
%
\cref{lem:kern_select}, which follows almost directly from the "sum property" of kernels,  highlights how each $\theta_V$ plays the role of a model selection parameter; if $\theta_V = 0$, then the effect $f_V = 0$. Hence, $\theta_V$ naturally leads to a variable selection procedure.
%
\begin{ncor} (non-linear variable selection)  \label{lem:kern_var_select}
Suppose $f^{(M)}(x)  = \sum_{m=1}^M \alpha_m k_{\theta}(x_m, x)$. Then, $f^{(M)}(x)$ functionally depends on the set of covariates $\{i: \exists V \subset [p], i \in V \text{ s.t. } \theta_V \neq 0\}$.
\end{ncor}

If we can somehow learn the kernel hyperparameters $\theta$ (e.g., using cross-validation), then we can find what covariates $\bar{f}_{\theta}$ depends on using \cref{lem:kern_var_select}. For these selected covariates, we can use \cref{lem:kern_select} to report any non-zero effects of interest, or report the full (estimated) functional ANOVA decomposition of $\bar{f}_{\theta}$. Unfortunately, evaluating $k_{\theta}$ once takes  $O(p^Q)$ time to compute on a pair of points in general. Hence, computing and inverting $ (K_{\theta} + \lambda I_{N \times N})^{-1} Y$ in \cref{eq:kern_ridge} takes $O(p^Q N^2)$ time and $O(N^3)$ time, respectively. To reduce this computational intractability, we introduce additional low-dimensional structure in $\theta$ and $k_V$. 



%  We start by assuming product measure and then develop a method that sits on top of everything to re-express fit to general measure.  
%
%Due to the curse-of-dimensionality, estimating higher-order effects depends exponentially (in terms of number of datapoints) for fixed precion. High-order effects are also harder to interpret. For these reasons, we assume in the main body and our experiments that $Q=2$ to simplify notation. We leave the general $Q$ case to the Appendix. 
%
%Our full procedure consists of three parts: (1) a new model that assumes product measure, (2) an efficeient method to perform variable selection and estimation in this model, and (3) a way to generalize and re-express fit in terms of arbitrary measure.
  
 
\subsection{Sparse Kernel Interaction Model} 
 We solve \cref{eq:kern_ridge} and fit the kernel hyperparameters $\{\theta_V\}$ to induce sparsity  in $O(pQN^2 + N^3)$ time. The key idea to make inference scale linearly with dimension is assuming low-dimensional structure in $\theta_V$. Specifically, we introduce auxiliary parameters $\kappa \in \R^p$ and $\eta \in \R^{Q + 1}$ such that $\theta_V = \prod_{i \in V} \eta_{|V|}^2 \kappa_i^2$. This factorization not only reduces the cost to solve \cref{eq:kern_ridge} but also enables us to perform variable selection in time \emph{linear} in dimension. In particular, $\theta_V$ equals 0 whenever there exists an $i \in V$ such that $\kappa_i = 0$. Hence, by \cref{lem:kern_var_select}, it suffices to return the non-zero components of $\kappa$ instead of scanning all $O(p^Q)$ number of $\{\theta_V\}$ terms for variable selection.
 
In addition to the low-dimensional structure in $\theta_V$,  our trick to solve  \cref{eq:kern_ridge} fast requires that the kernel $k_V(x, \tilde{x})$ in \cref{def:model_select_kernel} factorizes as a product of one-dimensional kernels: $k_V(x, \tilde{x}) =  \prod_{i \in V} k_i(x_i, \tilde{x}_i)$, where $k_i$ is the reproducing kernel for $\hilb_i^o$ in \cref{eq:orth_hilb}. Since our assumption that $k_V(x, \tilde{x}) =  \prod_{i \in V} k_i(x_i, \tilde{x}_i)$ only holds for independent covariates or when $Q < 2$, we show how to extend our procedure to the general $\mu$ case in \cref{sec:extend_gen_measure}. The main idea is to perform variable selection and estimation with respect to $\mu_{\tens}$ (so that we can use our efficient inference techniques for product measure), and then use a change of basis formula to re-express the fit. We start by motivating our choice of kernel from the hierarchical Bayesian formulation in \cref{sec:hierch_bayes_model}.  \\

\noindent \textbf{SKIM-FA Model Motivation}. 
We let $\eta_q$ play the role of quantifying the overall strength of $q$-way interactions. We construct $\kappa$ so that $\kappa_i$ plays the role of a "variable importance" measure for covariate $x_i$. Intuitively, a variable derives more "importance" if it has stronger main or interaction effects. Based on this intuition, we pick $\kappa_i$ to control the prior variance of both the main effects and interactions involving $x_i$. Hence, if it turns out an effect involving $x_i$ is strong, the posterior of $\kappa_i$ will place high-probability at large values (i.e., indicating that covariate $x_i$ has high "importance"). Building on the work of previous sparse Bayesian interaction models \citep{sparse_bayes_pairwise,Curtis13fastbayesian, heirc_sparisty, kit, chipman_bayes_glm, george1993variable}, we propose the following prior on $\Theta_V$:
%
\begin{equation} \label{eq:skim_fa_weight}
	\begin{split}
			\Theta_{V} \mid \eta, \kappa &\sim \normal\left(0,  \eta_{|V|}^2 \prod_{i \in V} \kappa_i^2 \cdot I_{B_V} \times I_{B_V}\right).
	\end{split}
\end{equation}
% 
Notice that if $\kappa_i = 0$, then the prior variance of $\Theta_V$ equals 0 whenever $i \in V$. Consequently, all effects involving $x_i$ will equal 0. Hence, the sparsity pattern of $\kappa$ will allow us to perform variable selection. 

\begin{ndefn}  \label{def:skim_kern} A \emph{SKIM-FA kernel} is a kernel that can be written as 
%
\begin{equation*}
	k_{\text{SKIM-FA}}(x, \tilde{x}) = \sum_{V: |V| \leq Q} \left[  \eta_{|V|}^2 \prod_{i \in V} \kappa_i^2 \right] k_V(x, \tilde{x}).
\end{equation*}
% 
for some $\kappa \in \R^p$ and $\eta \in \R^{Q + 1}$. 
\end{ndefn}

\begin{nprop} \label{cor:skim_kern_ridge_equiv} For a SKIM-FA kernel, \cref{eq:gen_bayes_model} can be replaced by \cref{eq:skim_fa_weight} in \cref{prop:model_select_bayes}. 
\end{nprop}

\begin{proof}
Set $\theta_V =  \eta_{|V|}^2 \prod_{i \in V} \kappa_i^2$ in \cref{prop:model_select_bayes}.
\end{proof}

\noindent \textbf{Sparsity Inducing Prior.} To induce sparsity in $\kappa$ for variable selection, we pick a prior on $\kappa_i$ that equals the mixture of a discrete point mass at 0 and a Uniform(0, 1) random variable. Similar to a \emph{spike-and-slab} prior \citep{george1993variable}, the point mass at $0$ allows us to achieve exact sparsity. Unlike a spike-and-slab prior, however, we construct our prior so that we can still take gradients (and hence use continuous optimization techniques like gradient descent); see \cref{algo:learn_skim_hyp} for details. Our construction involves introducing another random variable $U_i$ so that
%
\begin{equation}
	\kappa_i = \frac{1}{1 - c} \max(U_i - c, 0), \ U_i \sim \text{Uniform}(0, 1).
\end{equation}
%
Then, $\pr(\kappa_i = 0) = c$. Otherwise, with probability $1 - c$, $\kappa_i \sim \text{Uniform}(0, 1)$. Hence, $c$ plays a similar role as a prior inclusion probability in a spike-and-slab prior. Since $\kappa_i$ is a deterministic function of $U_i$, it suffices to estimate $U_i$ instead; see \cref{sec:skim_fast} for details.  

%In use an $L_1$ penalty on $\theta_V$ to achieve sparsity. This corresponds to a Laplace prior on $\theta_V$. In light of ADD CORR REF, we use a particular prior on kappa to induce sparsity. This prior itself makes posterior supported on sparse models but importantly this prior plays well with our gradient descent optimizationn which we detail in next section.
 
\subsection{Fast Representation and Reporting with Product Measure} \label{sec:skim_fast}
Without additional structure, a SKIM-FA kernel takes $O(p^Q)$ time to evaluate on a pair of points; the sum in \cref{def:skim_kern} has $O(p^Q)$  terms.  We show how to compute SKIM-FA kernels in $O(pQ)$ time. To achieve this speedup, we assume independent covariates. Specifically, we assume $\mu = \mu_{\tens}$, where $\mu_{\tens}(x) \coloneqq \mu_1(x_1) \tens \mu_2(x_2) \cdots \tens \mu_p(x_p)$ and $\mu_j$ is the marginal distribution of $x_j$. In \cref{sec:extend_gen_measure}, we generalize to the non-independent case by building on the method described below.  

Since any Hilbert space of square-integrable functions of $x_V$ can be approximated arbitrarily well by taking tensor products of  one-dimensional Hilbert spaces by \citet{stone1994, projection_anova}, we make the following additional assumption:
%
\begin{nassum} \label{assum:tens_space} (Tensor product space) For all $V \subset [p]$ and $1 \leq |V| \leq Q$, $\hilb_V =  \bigotimes_{i \in V} \hilb_i$.
\end{nassum}
%
Under \cref{assum:tens_space} and the assumption that $\mu=\mu_{\tens}$, \citet{ss_anova} show that $\hilb_V^o = \bigotimes \hilb_{i}^o$; see \cref{eq:orth_hilb} for a definition of $\hilb_V^o$ and $\hilb_i^o$. Since $k_i$ is the reproducing kernel for $\hilb_{i}^o$,  $\prod_{i \in V} k_i$ is the reproducing kernel for $\hilb_V^o$ by the product property of kernels\footnote{In \cref{A:model_implement_details} we show how to construct the reproducing kernel $k_i$ for $\hilb_i^o$.} \citep{ss_anova}. Given this structure in $k_V$, we show how to compute SKIM-FA kernels orders of magnitude faster.
%
\begin{nthm} \label{thm:skim_fast_form}
Suppose  $k_V(x, \tilde{x}) = \prod_{ i \in V} k_i(x_i, \tilde{x}_i)$. Then,  
%
\begin{equation} \label{eq:skim_fast_form}
	\begin{split}
	& k_{\mathrm{SKIM-FA}}(x, \tilde{x}) = \sum_{q=1}^Q \eta_q^2 \bar{k}_q(x, \tilde{x}) \quad \mathrm{s.t.} \\
	& \bar{k}_q(x, \tilde{x}) = \frac{1}{q} \sum_{s=1}^q (-1)^{s+1} \bar{k}_{q-s}(x, \tilde{x}) k^s(x, \tilde{x}),  \quad \bar{k}_0(x, \tilde{x}) = 1, \\
	& k^s(x, \tilde{x}) = \sum_{i=1}^p \kappa_i^{2s} [k_i(x_i, \tilde{x}_i)]^s.
	\end{split}
\end{equation}
%
\end{nthm}
%
As we show in \cref{A:proofs}, the key to proving \cref{thm:skim_fast_form} is an old recursive kernel formula provided in \citet[pg. 199]{vapnik95}. From \cref{thm:skim_fast_form}, we have two corollaries. The first requires a short recursive argument; see \cref{A:proofs}. The second follows immediately by setting $Q=2$ into \cref{eq:skim_fast_form}.

\begin{ncor} \label{corr:skim_kern_time}
$k_{\mathrm{SKIM-FA}}(x, \tilde{x})$ takes $O(pQ)$ time to evaluate on a pair of points.
\end{ncor}

\begin{ncor}
Suppose $Q=2$. Then, $k_{\text{SKIM-FA}}(x, \tilde{x})$ equals
%
\begin{equation}
	.5 \eta_2^2 \left [\left( \sum_{i=1}^p \kappa_i^2 k_i(x_i, \tilde{x}_i) \right)^2 - \sum_{i=1}^p \kappa_i^4 [k_i(x_i, \tilde{x}_i)]^2  \right] + \eta_1^2 \sum_{i=1}^p \kappa_i^2 k_i(x_i, \tilde{x}_i) + \eta_0^2
\end{equation}
%
\end{ncor}


\noindent \textbf{Cross-Validation Loss and Optimization.} We conclude by deriving our method to fit the SKIM-FA kernel hyperparameters. Given the empirical success of cross-validation and its use in other functional ANOVA methods (e.g., as in \citet{ss_anova, cosso}), we also use cross-validation to select hyperparameters. Specifically, we would like to pick $U, \eta, \noisevar$ (where $\kappa_i =  \frac{1}{1 - c} \max(U_i - c, 0)$) by minimizing a leave-$M$-out cross validation loss:
%
\begin{equation} \label{eq:exact_leave_out}
	\begin{split}
	L(U, \eta, \noisevar) &= \frac{1}{{N \choose M}} \sum_{\substack{A: A \subset [N] \\|A| = N - M}} \left[ \frac{1}{M} \sum_{m \in A} (y^{(m)} - \bar{f}_A(x^{(m)}))^2 \right], \\
									&=\E_{A \sim \pi} \left[  \frac{1}{M} \sum_{m \in A} (y^{(m)} - \bar{f}_A(x^{(m)}))^2 \right]
	\end{split}
\end{equation}
%
where $\bar{f}_A$ equals the kernel ridge regression fit in \cref{eq:kern_ridge} using the subset of datapoints in $A$ and $\pi$ equals the uniform distribution over all $N-M$ sized partitions of $[N]$. 

Since the gradient of $L(U, \eta, \noisevar)$ exists\footnote{Although $\frac{1}{1 - c} \max(U_i - c, 0)$ is not differentiable at $c$, we may instead take the subgradient. To compute gradients, we use the automatic differentiation library \texttt{PyTorch}.},  we can minimize \cref{eq:exact_leave_out} using gradient descent. However, this loss is computationally intensive; we need to solve \cref{eq:kern_ridge} ${N \choose M}$ times in order to take a single gradient descent step. Instead, we approximate \cref{eq:exact_leave_out} by using Monte Carlo cross validation. Specifically, we randomly draw a single $A$ from $\pi$ in \cref{eq:exact_leave_out} and use the mean-squared prediction error of $\bar{f}_A$ to estimate \cref{eq:exact_leave_out}. Then, this estimate leads to an unbiased estimate of \cref{eq:exact_leave_out}, and hence the gradient of $L(U, \eta, \noisevar)$. We summarize our full procedure in \cref{algo:learn_skim_hyp}. Note that in \cref{algo:learn_skim_hyp} we do not minimize over $U$ but instead over $\tilde{U}$, where $U_i = \frac{\tilde{U}_i^2}{\tilde{U}_i^2 + 1}$.  Since the range of $ \frac{\tilde{U}_i^2}{\tilde{U}_i^2 + 1}$ equals $(0, 1)$ when $\tilde{U}_i$ varies over all of $\R$, we can optimize $\tilde{U}_i$ over an unconstrained domain.
 
 \begin{algorithm}
    \caption{Learn SKIM-FA Kernel Hyperparameters and Kernel Ridge Weights}
    \label{algo:learn_skim_hyp}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        %\Procedure{LearnHyp}{$D$, $Q$, $c$, $\{k_i\}_{i=1}^p$, $M$, $\gamma$, $T$} where $D$ equals the observed data, $Q$ the highest order effect,  $c$ cutoff in ADD REF, $\{k_i\}_{i=1}^p$ univariate mean-zero kernels, $M$ the cross-validation fold size, $\gamma$ the learning rate, $T$ the number of gradient descent steps 
         \Procedure{LearnKernHyp}{$M$, $\gamma$, $T$} %$M$ the cross-validation fold size, $\gamma$ the learning rate, $T$ the number of gradient descent steps 

		\State For all $i  \in [p]$, set $\tilde{U}_i^{(0)} = 1$
		
		\State For all $q  \in [Q]$, set $\eta_q^{(0)} = 1$
		
		\State $\sigma^{(0)}_{\text{noise}} = \sqrt{.5\var(Y)}$ \Comment{Initialize noise variance as half of the response variance}
		
		\State $\tau^{(0)} = (\tilde{U}, \eta_q^{(0)},\sigma^{(0)}_{\text{noise}})$

            \For{$t \in 1:T$} \Comment{Update parameters via gradient descent}
            		\State{Randomly select $N-M$ datapoints and collect  covariates and responses in $X_A$, $Y_A$}
            		\State $U_i^{(t)} = \frac{[\tilde{U}_i^{(t)}]^2}{[\tilde{U}_i^{(t)}]^2 + 1}, i \in [p]$
            		
            		\State $\kappa_i^{(t)} = \max(U_i^{(t)} - c, 0), i \in [p]$
            		
            		\State Compute kernel matrix $K_{\tau}^A$, where $[K_{\tau}^A]_{ij} = k_{\text{SKIM-FA}}(X^A_i, X^A_j)$ via \cref{eq:skim_fast_form}
            		
            		\State Let $f_A$ equal the solution of \cref{eq:kern_ridge} with $\lambda = [\sigma^{(t)}_{\text{noise}}]^2$, $K = K_{\tau}^A$, $Y = Y_A$
            		
            		\State $L = \frac{1}{M} \sum_{n \in A^c} (y^{(n)} - f_A(x^{(n)}))^2$
            		
            		\State $\tau^{(t+1)} = \tau^{(t)}  - \gamma \nabla_{\tau^{(t)}} L$ \Comment{Compute gradients via an automatic differentiation library}
            		            		               
            \EndFor 
            
            \State Compute $\alpha^{(T)}$, the kernel ridge regression weights found by solving \cref{eq:kern_ridge} using all $N$ datapoints with SKIM-FA hyperparameters equal to $\kappa^{(T)}, \eta^{(T)}, \sigma^{(T)}_{\text{noise}}$
                                 
            \State \textbf{return} $\kappa^{(T)}, \eta^{(T)}, \sigma^{(T)}_{\text{noise}}, \alpha^{(T)}$
            
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

 \begin{algorithm}
    \caption{SKIM-FA Variable Selection}
    \label{algo:var_select}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        %\Procedure{LearnHyp}{$D$, $Q$, $c$, $\{k_i\}_{i=1}^p$, $M$, $\gamma$, $T$} where $D$ equals the observed data, $Q$ the highest order effect,  $c$ cutoff in ADD REF, $\{k_i\}_{i=1}^p$ univariate mean-zero kernels, $M$ the cross-validation fold size, $\gamma$ the learning rate, $T$ the number of gradient descent steps 
         \Procedure{VarSelect}{$\kappa$}
            \State \textbf{return} $ \{i: \kappa_i \neq 0 \} $
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

 \begin{algorithm}
    \caption{Estimated functional ANOVA effect $\bar{f}_V$ of $\bar{f}_{\theta}$ with respect to $\mu_{\tens}$}
    \label{algo:orth_effects}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        %\Procedure{LearnHyp}{$D$, $Q$, $c$, $\{k_i\}_{i=1}^p$, $M$, $\gamma$, $T$} where $D$ equals the observed data, $Q$ the highest order effect,  $c$ cutoff in ADD REF, $\{k_i\}_{i=1}^p$ univariate mean-zero kernels, $M$ the cross-validation fold size, $\gamma$ the learning rate, $T$ the number of gradient descent steps 
         \Procedure{OrthEffects}{$V$, $\alpha$, $\kappa$, $\eta$, $\alpha$} %where $\alpha$ equals the fitted kernel ridge regression weights

		\State $\theta_V = \eta_{|V|}^2 \prod_{i \in V} \kappa_i^2$
                      
            \State \textbf{return} $\bar{f}_V(\cdot) = \theta_V \sum_{n=1}^N \alpha_n k_V(x^{(n)}, \cdot)$ 
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{nprop} \label{prop:grad_descent}
Suppose $\kappa_i^{(t)} = 0$ at some iteration $t$ in \cref{algo:learn_skim_hyp}. Then, for all subsequent iterations $t' \geq t$, $\kappa_i^{(t')} = 0$. 
\end{nprop}
%\begin{proof}
% If at any gradient descent iteration $\nabla_{\kappa_i} L$ is large (i.e., the loss increases significantly by putting more importance to covariate $i$), $\tilde{\kappa_i}$ will fall below $\lambda$. In the next gradient step, the derivative with respect to $\tilde{\kappa}_i$ will be zero due to the indicator term. Hence, covariate $i$ will foreover be pruned off from the model since the gradient will remain at $0$ at all subsequent iterations. 
%\end{proof}

Based on \cref{prop:grad_descent}, we may  view \cref{algo:learn_skim_hyp} as a gradient-based analogue of backward stepwise regression; we start with the full saturated model by initializing all $\tilde{U}_i = 1$ (and consequently all $\kappa_i > 0$). Then, we keep pruning off covariates the longer we run gradient descent. We demonstrate empirically in \cref{sec:experiments} that the actual data-generating covariates remain while the irrelevant covariates get pruned off. Once we have found the kernel hyperparameters from \cref{algo:learn_skim_hyp}, \cref{algo:var_select} and \cref{algo:orth_effects} show how to perform variable selection and recover the effects, respectively. Both \cref{algo:var_select} and \cref{algo:orth_effects} follow directly from \cref{lem:kern_var_select} and \cref{lem:kern_select}. 


\subsection{Fast Reporting with General Measures} \label{sec:extend_gen_measure}

We conclude by extending our procedure to the general $\mu$ case when $Q=2$. We start by motivating why this extension is important. \\

\noindent \textbf{Pathologies with Product Measure.} Even though $\mu_{\tens}$ has the same 1D marginal distributions as  $\mu$,  we prove that the functional ANOVA decomposition of an $f \in \hilb$ can be \emph{arbitrarily} different depending on the choice of measure. We prove this claim by showing something stronger, namely that the intercepts between two functional ANOVA decompositions can be arbitrarily far apart.
%
\begin{nprop} \label{lem:arb_far_intercept}
For any $\Delta > 0$, there exists a probability measure $\mu$ and square-integrable $f$ such that the relative difference
%
\begin{equation*}
	\frac{| f_{\emptyset}^{\mu} - f_{\emptyset}^{\mu_{\tens}} |}{ |f_{\emptyset}^{\mu}|} > \Delta, \quad \text{where} \quad f_{\emptyset}^{\mu} =  \E_{\mu} f(X) \quad \text{and} \quad f_{\emptyset}^{\mu_{\tens}} =  \E_{\mu_{\tens}} f(X).
\end{equation*}
%
\end{nprop}
%
\begin{figure}
        \centering
        \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \includegraphics[width=\textwidth]{./figures/orth_example.png}
            % {{\small Positively Correlated Gene}}    
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.4\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{./figures/corr_example.png}
        \end{subfigure}
        	\caption{The colors denote the contour plot of the function $f^*(x_1, x_2) = x_1 x_2$. Darker green indicates more larger values while darker red indicates stronger negative values. The gray solid lines in the left and right hand figures represent the density contours of $\mu_{\tens}$ and $\mu$ in \cref{ex:prod_measure_issue}, respectively.} \label{fig:toy_prod_measure_issue}
\end{figure}
%
To build intuition for \cref{lem:arb_far_intercept}, and motivate using $\mu$ instead of $\mu_{\tens}$ to compute the functional ANOVA decomposition, consider the following toy example.
\begin{nexa} \label{ex:prod_measure_issue}
Suppose $f^*(x_1, x_2) = x_1 x_2$, where $x_1$ could represent exercise, $x_2$ protein consumption, and $f^*(x_1, x_2)$ the expected cardiovascular health of an individual who consumes $x_1$ grams of protein and exercises $x_2$ times per week. Suppose exercise and protein consumption are positively correlated and that $\mu$ equals a multivariate Gaussian distribution with mean zero, unit covariance, and correlation equal to $.9$. Then, $\mu_{\tens}$ equals a multivariate Gaussian distribution with mean zero, unit covariance but correlation equal to $0$. Suppose we   report the intercept $f_{\emptyset}$ to summarize the typical cardiovascular health in the population. In the functional ANOVA decomposition of $f^*$ with respect to $\mu$, $f_{\emptyset} = \E_{\mu}[f^*] =  \E_{\mu}[f^* + \epsilon] = \E_{\mu}[Y] \approx .89$. Hence, this intercept has the  interpretation as the average cardiovascular health in the population. If we instead use $\mu_{\tens}$, then $f_{\emptyset} = \E_{\mu_{\tens}} f^* = 0 \neq  \E_{\mu}[f^*]$. In this case, it is not clear how to interpret this intercept; $\mu_{\tens}$ averages the regression surface $f^*$ over individuals who rarely occur in the actual population (e.g., those who exercise very frequently but not not consume much protein); see also \cref{fig:toy_prod_measure_issue} for a visualization. 
\end{nexa}


\noindent \textbf{Extension to General Measures.} 
When $Q=2$, we show how to find the functional ANOVA decomposition of an $f \in \hilb$ without assuming $\mu = \mu_{\tens}$. The key idea is to construct the model space $\hilb$ to only contain functions that are square-integrable with respect to both $\mu$ and $\mu_{\tens}$. Then, $\hilb$ can be decomposed in multiple ways:
%
\begin{align}
		\hilb &=  \bigoplus_{V: |V| \leq Q} \hilb_V  \\
				&= \bigoplus_{V: |V| \leq Q} \hilb^o_{V, \mu_{\tens}} \label{eq:orth_param} \\
				&=  \bigoplus_{V: |V| \leq Q} \hilb^o_{V, \mu} \label{eq:target_param}
\end{align}
%
where $\hilb^o_{V, \mu}$ and $\hilb^o_{V, \mu_{\tens}}$ denote the set of functions in $\hilb_V$ that are orthogonal to all  lower-order effects, where orthogonality is measured with respect to $\mu$ and $\mu_{\tens}$, respectively; see, also, \cref{eq:orth_hilb}. We estimate $f^*$ and perform variable selection by using the computationally convenient $\mu_{\tens}$ parameterization of $\hilb$ in \cref{eq:orth_param}. Hence, we show below that we can still use \cref{algo:learn_skim_hyp} to learn the SKIM-FA kernel hyperparameters fast, and compute $\bar{f}_{\theta} \in \hilb$. Instead of returning the functional ANOVA decomposition of  $\bar{f}_{\theta}$ with respect to $\mu_{\tens}$ using \cref{algo:orth_effects}, we instead develop a change-of-basis formula in \cref{thm:theo_proj}. In \cref{algo:change_basis}, we use this change-of-basis formula to compute the functional ANOVA decomposition of $\bar{f}_{\theta}$ with respect to $\mu$. \\

\noindent \textbf{Construction of $\hilb$.}
To ensure each function in  $\hilb_V$ is square-integrable with respect to $\mu_{\tens}$ and $\mu$, we assume that $\hilb_V$ is finite-dimensional. Since $\hilb_V = \bigotimes_{i \in V} \hilb_i$, $\hilb_V$ is finite-dimensional if and only if each $\hilb_i$ is finite dimensional\footnote{If $\hilb_i$ is not finite-dimensional, we can approximately any function arbitrarily well by setting $B_i$ sufficiently large since $\hilb_i$ is seperable; see, \citet{projection_anova}, for rates of convergence for different finite-basis approximations.}.
%In light of the issues with product measure raised in ADD REF, we extend our method to the general  $\mu$ case when $Q=2$. As we already stated before, the tensor product spaces in allow to approximate any Hilbert space of square-integrable functions well. However, when $\mu \neq \mu_{\tens}$, then $\hilb_V^o \neq \bigotimes_{i \in V} \hilb_i^o$ in general when $Q > 1$. Hence, $k_V \neq \prod_{i \in V} k_i$ which was critical to compute the SKIM-FA kernel efficiently in ADD REF. To still retain the ability to perform inference efficiently, we require that each $\hilb_i$ is finite-dimensional:
%
\begin{nassum} \label{assum:finite_dim}
For all $i \in [p]$ there exists a  $B_i < \infty$ and linearly independent set of continuous functions $\{ \phi_{ib} \}_{i=1}^{B_i}$ such that $\hilb_i =\text{span}\{1, \phi_{i1}, \cdots, \phi_{iB_i} \}$ and $\Phi_i = [ \phi_{i1}, \cdots,  \phi_{iB_i}]^T$.% and $\E_{\mu_i}[ \phi_{ib}(x_i)] = 0$.
\end{nassum}
%
%\begin{nlem}
%Under \cref{assum:finite_dim}, $\hilb_i^o = \text{span}\{\phi_{i1}, \cdots, \phi_{iB_i} \}$. Furthermore, $k_i(x_i, \tilde{x}_i) = \inner{\Phi_i(x_i)}{\Phi_i(\tilde{x}_i)}$ is the reproducing kernel of $\hilb_i^o$, where $\Phi_i(x_i) = [\phi_{i1}(x_i), \cdots, \phi_{iB_i}(x_i)]$.
%\end{nlem}
%
%In general, if $\hilb_i$ is not finite-dimensional, we can approximately any function well by setting $B_i$ sufficiently large since $\hilb_i$ is seperable; see, \citet{projection_anova}, for rates of convergence for different finite-basis approximations. Then, under this assumption we can construct $\hilb$ to satisfy ADD REF. %In general,  often set $B$ small (e.g., equal to 5 or 10). For example, if you put a knot at each of decile in a B-spline, then number of basis functions equals 10.

\begin{nlem} \label{eq:universal_space}
Under \cref{assum:tens_space} and \cref{assum:finite_dim}, any $f \in \hilb$ is square-integrable with respect to any probability measure.  
\end{nlem}

By \cref{eq:universal_space}, we may decompose $\hilb$ as in \cref{eq:orth_param} and \cref{eq:target_param}. Following the same argument as in \cref{sec:skim_fast}, $\prod_{i \in V} k_i$ is the reproducing kernel for  $\hilb^o_{V, \mu_{\tens}}$. Hence, we can still run \cref{algo:learn_skim_hyp} to efficiently learn the SKIM-FA kernel hyperparameters and compute the kernel ridge regression estimate $\bar{f}_{\theta} \in \hilb$.  \cref{thm:theo_proj} below relates the functional ANOVA of $\bar{f}_{\theta}$ with respect to $\mu_{\tens}$ (which we can recover from \cref{algo:orth_effects}) to one with respect to $\mu$. From this relation, we develop \cref{algo:change_basis} to perform this change-of-basis in practice, and prove its correctness in \cref{prop:change_basis_correct}.  


%The first construction writes $\hilb$ as a direct sum of component spaces that satisfity the orthogonality constraits in ADD REF with respect to  $\mu_{\tens}$. We write this as $\hilb_{V, \mu_{\tens}}^o$.  The other writes  $\hilb$ as a direct sum of component spaces that satisfity the orthogonality constraits in ADD REF with respect to  $\mu$. We write this as $\hilb_{V, \mu}^o$. Since either parameterization spans the same model space $\hilb = \bigoplus  \hilb_{V, \mu_{\tens}}^o =  \bigoplus  \hilb_{V, \mu}^o$, we can use the computationall convenient $\mu_{\tens}$ parameterization to fit the kernel hyperparameters via ADD REF. Since variable selection just depends on $f$ we can still peform variable selection. We can also use the mean estimate in ADD REF.   Hence, we can estimate the aggregate sum of effects (i.e., mean function) of $f^*$ and perform variable selection via ADD REFs. Once, we have that, we can re-express the fit into the basis with respect to a functional ANOVA with respect to $\mu$. We conclude by showing how to theoretically perform this change of basis and the provide a practical (Monte Carlo) algorithm to actually do it in ADD REF.

\begin{nthm} \label{thm:theo_proj}
Suppose $Q=2$ and that \cref{assum:tens_space} and \cref{assum:finite_dim} hold. For $f \in \hilb$, let
%
\begin{equation*}
	\begin{split}
		f &= f_{\emptyset}^{\mu_{\tens}} + \sum_{i=1}^p f_{\{ i\}}^{\mu_{\tens}} + \sum_{i,j=1}^p f_{\{ i, j \}}^{\mu_{\tens}} \\
			&= f_{\emptyset}^{\mu} + \sum_{i=1}^p f_{\{ i\}}^{\mu} + \sum_{i,j=1}^p f_{\{ i, j \}}^{\mu}
	\end{split}
\end{equation*}
%
be the functional ANOVA decompositions of $f$ with respect to $\mu_{\tens}$ and $\mu$, respectively. Then, there exists unique coefficients, $\Psi_{ij}^i \in \R^{1 \times B_i}, \Psi_{ij}^j  \in \R^{1 \times B_j}, \Psi_{ij}^{0} \in \R$, such that
%
\begin{equation}
	 \begin{split} \label{eq:change_basis}
	 	 f_{\{ i, j \}}^{\mu}(x_i, x_j) &=  f_{\{ i, j \}}^{\mu_{\tens}}(x_i, x_j) - [\Psi_{ij}^i \Phi_i(x_i) +  \Psi_{ij}^j \Phi_j(x_j) + \Psi_{ij}^{0}] \\
	 	f_{\{ i \}}^{\mu}(x_i) &=f_{\{ i \}}^{\mu_{\tens}}(x_i) + \sum_{j > i} \Psi_{ij}^i \Phi_i(x_i) + \sum_{j < i} \Psi_{ji}^{i} \Phi_i(x_i)  \\
	 	f_{\emptyset}^{\mu} &= f_{\emptyset}^{\mu_{\tens}} + \sum_{i < j} \Psi_{ij}^{0},
	 \end{split}
\end{equation}
%
where $\Phi_i$ denotes the (finite-dimensional) feature map in \cref{def:model_select_kernel}.
\end{nthm}
%
We prove \cref{thm:theo_proj} in \cref{A:proofs}. It remains to show how we can actually compute each $\Psi_{ij}^i$ in \cref{thm:theo_proj}. In \cref{algo:change_basis}, we estimate $\Psi_{ij}^i$  using a Monte Carlo approach. 


 \begin{algorithm}
    \caption{Change of Basis Formula for Finite Dimensional Model Selection Kernels}
    \label{algo:change_basis}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
         \Procedure{ReExpressEffect}{$\alpha$, $k_{\theta}$, $W$, $\mu$}  
         	\State Compute $ f_{\{ i, j \}}^{\mu_{\tens}} , f_{\{ i \}}^{\mu_{\tens}}, f_{\emptyset}^{\mu_{\tens}}$ using \cref{algo:orth_effects}
			\State For $1 \leq w \leq W$ randomly sample $x^{(w)} \iid \mu$     
			\State Compute $X_{ij} = [\Phi_i(x^{(1)}_i) \cdots \Phi_i(x^{(W)}_i) \ \Phi_j(x^{(1)}_j) \cdots \Phi_j(x^{(W)}_j)]^T$
			\State Compute  $f_{ij, W}^{\mu_{\tens}} = [f_{\{ i, j \}}^{\mu_{\tens}}(x^{(1)}_i,  x^{(1)}_j) \cdots f_{\{ i, j \}}^{\mu_{\tens}}(x^{(W)}_i,  x^{(W)}_j)]^T$
			\State Compute $[\hat{\Psi}_{ij}^i \ \hat{\Psi}_{ij}^j]^T = (X_{ij}^T X_{ij})^{-1} X_{ij}^T f_{ij, W}^{\mu_{\tens}}$ \Comment{Least-squares projection}
			\State Compute $\hat{f}_{\{ i, j \}}^{\mu} =  f_{\{ i, j \}}^{\mu_{\tens}} - [\hat{\Psi}_{ij}^i \Phi_i^T(\cdot) +  \hat{\Psi}_{ij}^j \Phi_j^T(\cdot) + \Psi_{ij}^{0}]$
			\State Compute $\hat{f}_{\{ i \}}^{\mu} =f_{\{ i \}}^{\mu_{\tens}} + \sum_{j > i} \hat{\Psi}_{ij}^i \Phi_i(\cdot) + \sum_{j < i} \hat{\Psi}_{ji}^{i} \Phi_i(\cdot)$ 
			\State Compute $\hat{f}_{\emptyset}^{\mu} = f_{\emptyset}^{\mu_{\tens}} + \sum_{i < j} \hat{\Psi}_{ij}^{0}$
            \State \textbf{return} $\hat{f}_{\{ i, j \}}^{\mu}, \hat{f}_{\{ i \}}^{\mu}, \hat{f}_{\emptyset}^{\mu} $
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{nprop} \label{prop:change_basis_correct}
Let $W \rightarrow \infty$ in \cref{algo:change_basis}. Then, the components returned from \cref{algo:change_basis} converge to the decomposition in \cref{eq:change_basis}.
\end{nprop}



==> tables/synthetic/all_effects.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{lscape}
\begin{landscape}
\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
\textbf{p} & \textbf{setting} & \textbf{Method} & \textbf{\begin{tabular}[c]{@{}c@{}}Correct \\ Selected \\ SSE (Main)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Correct \\ Not Selected \\ SSE (Main)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Wrong\\ Selected SSE\\ (Main)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Correct\\ Selected \\ SSE (Pair)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Correct\\ Not Selected \\ SSE (Pair)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Wrong\\ Selected \\ SSE (Pair)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Total \\ SSE\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Total SSE / \\ Signal \\ Variance\end{tabular}} \\ \midrule
250        & EQUAL            & SKIM-FA         & 1.62                                                                               & 0.00                                                                                   & 0.08                                                                           & 0.52                                                                              & 0.00                                                                                  & 0.17                                                                            & 2.39                                                          & 0.12                                                                               \\
250        & EQUAL            & SPAM-2Stage     & 1.63                                                                               & 0.00                                                                                   & 1.72                                                                           & 8.84                                                                              & 0.00                                                                                  & 0.11                                                                            & 12.30                                                         & 0.62                                                                               \\
250        & EQUAL            & MARS            & 10.11                                                                              & 0.00                                                                                   & 3.36                                                                           & 4.19                                                                              & 0.00                                                                                  & 7.33                                                                            & 25.00                                                         & 1.25                                                                               \\
           &                  &                 &                                                                                    &                                                                                        &                                                                                &                                                                                   &                                                                                       &                                                                                 &                                                               &                                                                                    \\
500        & EQUAL            & SKIM-FA         & 1.52                                                                               & 0.00                                                                                   & 0.00                                                                           & 0.41                                                                              & 0.00                                                                                  & 0.00                                                                            & 1.93                                                          & 0.10                                                                               \\
500        & EQUAL            & SPAM-2Stage     & 1.62                                                                               & 0.00                                                                                   & 3.74                                                                           & 2.16                                                                              & 0.00                                                                                  & 5.47                                                                            & 12.99                                                         & 0.65                                                                               \\
500        & EQUAL            & MARS            & 9.30                                                                               & 0.00                                                                                   & 4.19                                                                           & 5.45                                                                              & 0.00                                                                                  & 8.57                                                                            & 27.52                                                         & 1.38                                                                               \\
           &                  &                 &                                                                                    &                                                                                        &                                                                                &                                                                                   &                                                                                       &                                                                                 &                                                               &                                                                                    \\
1000       & EQUAL            & SKIM-FA         & 1.54                                                                               & 0.00                                                                                   & 0.00                                                                           & 0.29                                                                              & 0.00                                                                                  & 0.00                                                                            & 1.82                                                          & 0.09                                                                               \\
1000       & EQUAL            & SPAM-2Stage     & 1.67                                                                               & 0.00                                                                                   & 1.07                                                                           & 0.41                                                                              & 0.00                                                                                  & 2.16                                                                            & 5.31                                                          & 0.27                                                                               \\
1000       & EQUAL            & MARS            & 7.13                                                                               & 0.00                                                                                   & 4.12                                                                           & 3.61                                                                              & 0.00                                                                                  & 3.56                                                                            & 18.43                                                         & 0.92                                                                               \\
           &                  &                 &                                                                                    &                                                                                        &                                                                                &                                                                                   &                                                                                       &                                                                                 &                                                               &                                                                                    \\
250        & MAIN ONLY        & SPAM-2Stage     & 2.77                                                                               & 0.00                                                                                   & 1.99                                                                           & 0.00                                                                              & 0.00                                                                                  & 0.08                                                                            & 4.84                                                          & 0.24                                                                               \\
250        & MAIN ONLY        & MARS            & 0.48                                                                               & 0.00                                                                                   & 1.71                                                                           & 0.00                                                                              & 0.00                                                                                  & 3.21                                                                            & 5.39                                                          & 0.27                                                                               \\
250        & MAIN ONLY        & SKIM-FA         & 2.75                                                                               & 4.02                                                                                   & 0.00                                                                           & 0.39                                                                              & 0.00                                                                                  & 0.00                                                                            & 7.16                                                          & 0.36                                                                               \\
           &                  &                 &                                                                                    &                                                                                        &                                                                                &                                                                                   &                                                                                       &                                                                                 &                                                               &                                                                                    \\
500        & MAIN ONLY        & SPAM-2Stage     & 2.82                                                                               & 0.00                                                                                   & 1.25                                                                           & 0.00                                                                              & 0.00                                                                                  & 0.04                                                                            & 4.11                                                          & 0.21                                                                               \\
500        & MAIN ONLY        & SKIM-FA         & 2.75                                                                               & 0.00                                                                                   & 0.49                                                                           & 0.12                                                                              & 0.00                                                                                  & 1.28                                                                            & 4.64                                                          & 0.23                                                                               \\
500        & MAIN ONLY        & MARS            & 0.65                                                                               & 0.00                                                                                   & 2.41                                                                           & 0.09                                                                              & 0.00                                                                                  & 2.53                                                                            & 5.69                                                          & 0.28                                                                               \\
           &                  &                 &                                                                                    &                                                                                        &                                                                                &                                                                                   &                                                                                       &                                                                                 &                                                               &                                                                                    \\
1000       & MAIN ONLY        & SPAM-2Stage     & 2.67                                                                               & 0.00                                                                                   & 0.78                                                                           & 0.00                                                                              & 0.00                                                                                  & 0.01                                                                            & 3.46                                                          & 0.17                                                                               \\
1000       & MAIN ONLY        & MARS            & 0.83                                                                               & 0.00                                                                                   & 2.09                                                                           & 0.00                                                                              & 0.00                                                                                  & 3.23                                                                            & 6.15                                                          & 0.31                                                                               \\
1000       & MAIN ONLY        & SKIM-FA         & 2.70                                                                               & 8.10                                                                                   & 0.00                                                                           & 0.24                                                                              & 0.00                                                                                  & 0.00                                                                            & 11.03                                                         & 0.55                                                                               \\
           &                  &                 &                                                                                    &                                                                                        &                                                                                &                                                                                   &                                                                                       &                                                                                 &                                                               &                                                                                    \\
250        & WEAK MAIN        & SKIM-FA         & 0.45                                                                               & 0.00                                                                                   & 0.95                                                                           & 0.73                                                                              & 0.00                                                                                  & 0.77                                                                            & 2.89                                                          & 0.14                                                                               \\
250        & WEAK MAIN        & SPAM-2Stage     & 0.09                                                                               & 0.05                                                                                   & 2.22                                                                           & 10.72                                                                             & 7.73                                                                                  & 0.42                                                                            & 21.23                                                         & 1.06                                                                               \\
250        & WEAK MAIN        & MARS            & 11.71                                                                              & 0.00                                                                                   & 4.35                                                                           & 8.63                                                                              & 0.00                                                                                  & 5.71                                                                            & 30.40                                                         & 1.52                                                                               \\
           &                  &                 &                                                                                    &                                                                                        &                                                                                &                                                                                   &                                                                                       &                                                                                 &                                                               &                                                                                    \\
500        & WEAK MAIN        & SKIM-FA         & 0.69                                                                               & 0.00                                                                                   & 2.05                                                                           & 1.50                                                                              & 0.00                                                                                  & 1.37                                                                            & 5.61                                                          & 0.28                                                                               \\
500        & WEAK MAIN        & SPAM-2Stage     & 0.27                                                                               & 0.20                                                                                   & 4.09                                                                           & 0.00                                                                              & 19.46                                                                                 & 0.08                                                                            & 24.11                                                         & 1.21                                                                               \\
500        & WEAK MAIN        & MARS            & 0.37                                                                               & 0.15                                                                                   & 20.52                                                                          & 1.94                                                                              & 17.52                                                                                 & 19.08                                                                           & 59.59                                                         & 2.98                                                                               \\
           &                  &                 &                                                                                    &                                                                                        &                                                                                &                                                                                   &                                                                                       &                                                                                 &                                                               &                                                                                    \\
1000       & WEAK MAIN        & SKIM-FA         & 0.72                                                                               & 0.00                                                                                   & 1.37                                                                           & 0.61                                                                              & 0.00                                                                                  & 0.63                                                                            & 3.33                                                          & 0.17                                                                               \\
1000       & WEAK MAIN        & SPAM-2Stage     & 0.16                                                                               & 0.20                                                                                   & 6.69                                                                           & 0.00                                                                              & 18.33                                                                                 & 0.31                                                                            & 25.69                                                         & 1.28                                                                               \\
1000       & WEAK MAIN        & MARS            & 10.63                                                                              & 0.00                                                                                   & 5.31                                                                           & 6.61                                                                              & 0.00                                                                                  & 6.66                                                                            & 29.21                                                         & 1.46                                                                               \\ \bottomrule
\end{tabular}
\end{table}
\end{landscape}
